Types by Need (Extended Version)

A cornerstone of the theory of lambda-calculus is that intersection types characterise termination properties. They are a flexible tool that can be adapted to various notions of termination, and that also induces adequate denotational models. Since the seminal work of de Carvalho in 2007, it is known that multi types (i.e. non-idempotent intersection types) refine intersection types with quantitative information and a strong connection to linear logic. Typically, type derivations provide bounds for evaluation lengths, and minimal type derivations provide exact bounds. De Carvalho studied call-by-name evaluation, and Kesner used his system to show the termination equivalence of call-by-need and call-by-name. De Carvalho's system, however, cannot provide exact bounds on call-by-need evaluation lengths. In this paper we develop a new multi type system for call-by-need. Our system produces exact bounds and induces a denotational model of call-by-need, providing the first tight quantitative semantics of call-by-need.

==> local_macros.tex <==
%%%\usepackage{amssymb}

\let\proof\relax
\usepackage{amsmath}
\let\endproof\relax

\usepackage{mathtools}
\usepackage{xspace}
\usepackage{amsthm}
\usepackage{fancybox}
\usepackage{proof}
\usepackage{xcolor}
\usepackage{ifthen}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% SCATTERED-SOURCED DEFINITIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Comments
\newcommand{\ben}[1]{{\color{red} {#1}}}
\newcommand{\maico}[1]{{\color{blue} {#1}}}
\newcommand{\giulio}[1]{{\color{green} {#1}}}

\newcommand{\cbn}{{CbN}}

\newcommand{\col}{\mathtt{:}}
\newcommand\eqdef{ \coloneqq }
\newcommand\recdef{ \Coloneqq }
\renewcommand\l{\lambda}

\newcommand{\sm}{\setminus \!\!\! \setminus}

\newcommand{\mult}[1]{[ #1 ] }
\newcommand{\funresult}{{\tt fun}_\result}
\newcommand{\tderiv}{\Phi}
\newcommand{\tderivtwo}{\tderiv'}
\newcommand{\tderivthree}{\tderiv''}
\newcommand{\tderivfour}{\tderiv'''}
\newcommand{\oc}{\mathtt{!}}
\newcommand{\ax}{\mathtt{ax}}
\newcommand{\exder}{\triangleright}
\newcommand{\appresult}{{\tt app}_\result}
\newcommand{\tri}{\triangleright}
\newcommand\dom[1]{{\tt dom}({#1})}
\newcommand{\iz}{i_1}


\newcommand{\TCS}{{\tt TC }}
\newcommand{\PS}{{\tt P }}


\newcommand{\mabstype}{\mathtt{Abs}}
\newcommand{\abstype}{\mathtt{abs}}
\newcommand{\absp}[1]{\abstype(#1)}

\newcommand{\iI}{{i \in I}}
\newcommand{\jJ}{{j \in J}}
\newcommand{\kK}{{k \in K}}

\newcommand{\emm}{ [\,] }
\newcommand{\emptymset}{\emm}

\newcommand{\app}{{\tt app}}
\newcommand{\appsteps}{\app_\steps}
\newcommand{\appstepsi}{\app_{\steps1}}
\newcommand{\appstepsii}{\app_{\steps2}}

\newcommand{\tyjn}[4]{{#3} \vdash^{#1} #2{:}#4}
\newcommand{\tyjp}[4]{{#3} \vdash^{#1} #2{:}#4}

\newcommand{\garbage}{g}
\newcommand{\Garbage}{G}
\newcommand{\garbagetwo}{\garbage'}
\newcommand{\garbagethree}{\garbage''}
\newcommand{\garbagefour}{\garbage'''}

\newcommand{\Gam}{\Gamma}
\newcommand{\Del}{\Delta}

\newcommand{\steps}{b}
\newcommand{\esteps}{e}
\newcommand{\estepstwo}{\esteps'}
\newcommand{\estepsthree}{\esteps''}
\newcommand{\Steps}{B}
\newcommand{\ESteps}{E}
\newcommand{\stepstwo}{\steps'}
\newcommand{\stepsthree}{\steps''}
\newcommand{\stepsfour}{\steps'''}

\newcommand{\sig}{\sigma}
\newcommand{\type}{\sig}
\newcommand{\typetwo}{\rho}
\newcommand{\typethree}{\tau}
\newcommand{\typefour}{\type'}
\newcommand{\typefive}{\typetwo'}

\newcommand{\Spine}{\Result}
\newcommand{\spine}{\result}
\newcommand{\spinetwo}{\spine'}
\newcommand{\spinethree}{\spine''}
\newcommand{\spinefour}{\spine'''}

\newcommand{\mtype}{{\tt A}}
\newcommand{\mtypetwo}{{\tt B}}
\newcommand{\mtypethree}{{\tt C}}
\newcommand{\M}{\mtype}
\newcommand{\N}{\mtypetwo}

\newcommand{\tight}{{\tt tight}}
\newcommand{\nf}{\tight}
\newcommand{\mtight}{\mathtt{Tight}}
\newcommand{\tightpred}[1]{{\tt tight}({#1})}
\newcommand{\mtightpred}[1]{\mem-\tt{tight}({#1})}

\newcommand{\result}{r}
\newcommand{\Result}{R}
\newcommand{\resulttwo}{\result'}
\newcommand{\resultthree}{\result''}
\newcommand{\resultfour}{\result'''}

\newcommand{\precise}{tight\xspace}

\newcommand{\neutral}{{\tt neutral}}
\newcommand\neutralpr[1]{{\tt neutral}^{#1}}
\newcommand\neutralp[2]{\neutralpr{#2}(#1)}
\newcommand{\neutralpred}[1]{{\tt neutral}(#1)}

\newcommand{\minerttype}{{\tt Inert}}
\newcommand\inerttype{{\tt inert}}
\newcommand{\inertpr}[1]{\inerttype ^ {#1}}
\newcommand{\inertp}[2]{\inertpr{#2}({#1})}
\newcommand{\inertpred}[1]{\inerttype(#1)}

\newcommand\normalpr[1]{{\tt normal}^{#1}}
\newcommand\normalp[2]{\normalpr{#2}(#1)}
\newcommand{\normalsharp}[1]{{\tt normal}^{\#}(#1)}
\newcommand{\normalpred}[1]{{\tt normal}(#1)}

%%% Command for typing judgements.
\newcommand{\Deri}[4]{#2 \, \vdash^{#1} \, #3 \, \col \, #4}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% PREVIOUS DEFINITION IS INTENDED TO REPLACE THE FOLLOWING ONES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%\newcommand\Deribbase[5]{{#3}\ {\pmb\vdash}_{#2}^{#1} {#4}\  {:}\  {#5}}
%%%
%%%\newcommand{\Deribase}[1]{%
%%%  \def\DeribW[##1]{\Deribbase{##1}{#1}}%
%%%  \def\DeribWO{\Deribbase{}{#1}}%
%%%  \@ifnextchar[\DeribW\DeribWO%
%%%}
%%%\newcommand{\Deri}{%
%%%  \def\DeriW_##1{\Deribase{##1}}%
%%%  \def\DeriWO{\Deribase{}}%
%%%  \@ifnextchar_\DeriW\DeriWO%
%%%}

%%% Command for typing derivations expliciting its final judgement.
\newcommand{\FullDeri}[5]{#1 \, \exder \, #3 \, \vdash^{#2} \, #4 \, \col \, #5}

%%% Typing derivations for the tight constants type system
\newcommand{\FullDeriTCS}[5]{#1 \, \exder_{\TCS} \, #3 \, \vdash^{#2} \, #4 \, \col \, #5}

%%% Typing derivations for the pure type system
\newcommand{\FullDeriPS}[5]{#1 \, \exder_{\PS} \, #3 \, \vdash^{#2} \, #4 \, \col \, #5}

%%% Indexed typing derivation
\newcommand{\FullDeriI}[6]{#2 \, \exder_{#1} \, #4 \, \vdash^{#3} \, #5 \, \col \, #6}


%%%%%%%
%% SUBSTITUTIONS
%%%%%%%
\newcommand{\isub}[2]{\{#1/#2\}}
\newcommand{\esub}[2]{[#1/#2]}
\renewcommand{\esub}[2]{[#1 \backslash #2]}
\renewcommand{\isub}[2]{\{#1{\shortleftarrow}#2\}}
\renewcommand{\L}{{\tt L}}
\newcommand{\Lv}[1]{{\tt L}_{#1}}
\newcommand{\letexp}[3]{{\tt let}\ #1=#2\ {\tt in}\ #3}




%%%%%%%
%% SYMBOLIZED LETTERS
%%%%%%%
\newcommand{\ssym}{{\tt s}}
\newcommand{\osym}{o}
\newcommand{\oboxsym}{obox}
\newcommand{\vosym}{vo}
\newcommand{\lssym}{{\tt ls}}
\newcommand{\ls}{\lssym}
\newcommand{\lsvsym}{{\tt lsv}}
\newcommand{\lsv}{\lsvsym}
\newcommand{\gcsym}{{\tt gc}}
\newcommand{\Bsym}{{\tt B}}
\newcommand{\db}{{\tt dB}}
\newcommand{\Esym}{{\tt E}}
\newcommand{\esym}{{\mathtt e}}
\newcommand{\wsym}{{\mathtt w}}
\newcommand{\usym}{{\mathtt u}}
\newcommand{\msym}{{\mathtt m}}
\newcommand{\fsym}{{\mathtt f}}
\newcommand{\psym}{{\mathtt p}}

\newcommand{\csym}{{\tt c}}
%\newcommand{\wsym}{{\tt w}}
\newcommand{\vsym}{{\tt v}}



%%%%%%%
%% CALL-BY-VALUE
%%%%%%%

\newcommand{\cbv}{{CbV}}

\newcommand{\val}{v}
\newcommand{\valtwo}{w}
\newcommand{\valthree}{v'}
\newcommand{\valfour}{w'}

% call-by-value root rules
\newcommand{\rtodbv}{\rootRew{\db\vsym}}
\newcommand{\rtolsv}{\rootRew{\lssym\vsym}}
\newcommand{\rtolsvc}[1]{\stackrel{#1}{\mapsto}_{\lssym\vsym}}

% call-by-value contexts
\newcommand{\cbvctx}{E}
\newcommand{\cbvctxtwo}{\cbvctx'}
\newcommand{\cbvctxthree}{\cbvctx''}
\newcommand{\cbvctxfour}{\cbvctx'''}
\newcommand{\cbvctxp}[1]{\cbvctx\ctxholep{#1}}
\newcommand{\cbvctxtwop}[1]{\cbvctxtwo\ctxholep{#1}}
\newcommand{\cbvctxthreep}[1]{\cbvctxthree\ctxholep{#1}}
\newcommand{\cbvctxfourp}[1]{\cbvctxfour\ctxholep{#1}}






%%%%%%%%
% CbNeed
%%%%%%%%
\newcommand{\cbneed}{{CbNeed}}

\newcommand{\ndsym}{\mathtt{nd}}
\newcommand{\ndc}{\mathtt{N}}
\newcommand{\ndcb}{\ndc'}
\newcommand{\ndcbb}{\ndcb'}
\newcommand{\Lb}{\L'}
\newcommand{\hole}[1]{\langle #1 \rangle}
\newcommand{\chole}{\langle \, \rangle}

\newcommand{\ndfv}[1]{\mathtt{nfv}(#1)}

\newcommand{\sizend}[1]{\size{#1}_{\ndsym}}
\newcommand{\sizelsv}[1]{\size{#1}_{\lssym\vsym}}

\newcommand{\Nnf}{\mathtt{N}_\ndsym}
\newcommand{\NAnf}{\mathtt{A}_\ndsym}
\newcommand{\NBnf}{\mathtt{B}_\ndsym}
\newcommand{\NCnf}{\mathtt{C}_\ndsym}

\newcommand{\ptype}{P}
\newcommand{\ptypeb}{Q}
\newcommand{\ptypethree}{R}
\newcommand{\ntype}{N}
\newcommand{\ntypeb}{M}
\newcommand{\To}[2]{#1 \to #2}

\newcommand{\fun}{{\tt fun}}
\newcommand{\funsteps}{{\tt fun}_\steps}
\newcommand{\ES}{\text{ES}}
\newcommand{\gc}{\text{gc}}
\newcommand{\fungc}{\fun_{\gc}}
\newcommand{\ESgc}{\ES_{\gc}}
\newcommand{\appgc}{\app_{\gc}}

\newcommand{\ESresult}{\ES_{\result}}


\newcommand{\tolsv}{\Rew{\lssym\vsym}}
\newcommand{\tond}{\Rew{\ndsym}}
\newcommand{\klop}{{\tt K}}
\newcommand{\mm}[1]{[\! [ #1 ] \! ]}
\newcommand{\deft}[1]{{\bf #1}}
\newcommand{\bv}[1]{{\tt bv}(#1)}
\newcommand{\neb}{{\tt neb}}
\newcommand{\mem}{{\tt m}}
\newcommand{\putinctx}[2]{#1 \langle #2 \rangle }
\newcommand{\mctx}{{\tt M}}
\newcommand{\rrule}[1]{\mapsto_{#1}}
\newcommand{\eras}[3]{#1\ \mathcal{E}^{#3}\ #2} 
\newcommand{\erasvoid}{\mathcal{E}}
\newcommand{\trad}[1]{{\tt T}(#1)}

\newcommand{\vleaf}{\bullet}
\newcommand{\noleaf}{\star}
\newcommand{\aabs}[1]{{\tt a}(#1)}
\newcommand{\aapp}[2]{{\tt c}(#1,#2)}
\newcommand{\polcomp}[2]{\delta(#1,#2)}
\newcommand{\mute}{\mbox{close}}


%% LINEAR HEAD REDUCTION
\newcommand{\lhr}{LHR}
\newcommand{\tohl}{\multimap}
\newcommand{\tohldb}{\multimap_\db}
\newcommand{\tohlls}{\multimap_\lssym}
\newcommand{\rtohls}{\rootRew{{\tt h}\lssym}}

\renewcommand{\lhd}{{lhd}}
\newcommand{\lh}{\lhd}
\newcommand{\lsp}{\lhd}
\newcommand{\lspb}{(\lsp_\msym)}
\newcommand{\lsps}{(\lsp_{\esym})}
\newcommand{\lspe}{(\lsp_{\esym})}
\newcommand{\lspapp}{(\lsp_{@})}
\newcommand{\lspabs}{(\lsp_{\l})}
\newcommand{\lspsub}{(\lsp_{s})}
\newcommand{\lhb}{(\lh_\msym)}
\newcommand{\lhs}{(\lh_{\esym})}
\newcommand{\lhapp}{(\lh_{@})}
\newcommand{\lhabs}{(\lh_{\l})}
\newcommand{\lhsub}{(\lh_{s})}

\newcommand{\tolh}{\Rew{\lh}}
\newcommand{\tolsp}{\rightarrow_{\lsp}}
\newcommand{\lhsp}{\lsp}
\newcommand{\tolhb}{\Rew{\msym}}
\newcommand{\tolhs}{\Rew{\esym}}
\newcommand{\tolspe}{\Rew{\esym}}
\newcommand{\tolspb}{\Rew{\msym}}
\newcommand{\lhc}{{\tt H}}
\newcommand{\lhcb}{{\tt H '}}
\newcommand{\cwc}[1]{\langle  \! \langle    #1 \rangle  \! \rangle}





%%%%%%%
%% SUBSTITUTION CALCULUS
%%%%%%%
\newcommand{\lsub}{\l_{sub}}
\newcommand{\tolsub}{\Rew{\lsub}}
\newcommand{\rtodb}{\rootRew{\db}}
\newcommand{\rtos}{\rootRew{\ssym}}
\newcommand{\tos}{\Rew{\ssym}}
\newcommand{\todbp}[1]{\Rew{\db#1}}
%\newcommand{\todb}{\todbp{}}%{\rightsquigarrow}
\newcommand{\todb}{\Rew{\db}}




%%%%%%%
%% ABBREVIATIONS
%%%%%%%
\renewcommand{\l}{\lambda}
\newcommand{\cf}{\emph {c.f.}\xspace}
\newcommand{\ie}{\emph {i.e.}\xspace}
\newcommand{\eg}{\emph {e.g.}\xspace}
\newcommand{\ih}{\emph{i.h.}\xspace}
\newcommand{\fv}[1]{{\tt fv}(#1)}
\newcommand{\fvvoid}{{\tt fv}}
\newcommand{\mfv}[1]{{\tt mfv}(#1)}
\newcommand{\nmfv}[1]{{\tt nmfv}(#1)}
\newcommand{\mfvvoid}{{\tt mfv}}
\newcommand{\ifv}[1]{\ifvvoid(#1)}
\newcommand{\ofv}[1]{\ofvvoid(#1)}
\newcommand{\ifvvoid}{{\tt ifv}}
\newcommand{\ofvvoid}{{\tt ofv}}
\newcommand{\hfv}[1]{{\tt hfv}(#1)}

\newcommand{\linlogic}{linear logic\xspace}
\newcommand{\Linlogic}{Linear logic\xspace}
\newcommand{\pn}{proof net\xspace}
\newcommand{\Pn}{Proof net\xspace}
\newcommand{\pns}{proof nets\xspace}
\newcommand{\Pns}{Proof nets\xspace}



%%%%%%%
%% REWRITING RELATION
%%%%%%%
\newcommand{\Rew}[1]{\xrightarrow{}_{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% PREVIOUS DEFINITION IS INTENDED TO REPLACE THE FOLLOWING ONES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\newcommand{\Rew}[1]{%
%%%  \def\RewW[##1]{\Rewbase[##1]{#1}{}}%
%%%  \def\RewWO{\Rewbase{#1}{}}%
%%%  \@ifnextchar[\RewW\RewWO%
%%%  }
  


  
%%%%%%%
%% REWRITING RELATIONS
%%%%%%%
\newcommand{\rootRew}[1]{\mapsto_{#1}}



%%%%%%%
%% TERMS AND VARIABLES
%%%%%%%

\newcommand{\lterms}{\Lambda}
\newcommand{\ltermslsc}{\Lambda_{{\tt lsc}}}
\newcommand{\la}[1]{\lambda #1.}

\newcommand{\tm}{t}
\newcommand{\tmtwo}{p}
\newcommand{\tmthree}{u}
\newcommand{\tmfour}{q}
\newcommand{\tmfive}{m}
\newcommand{\tmsix}{r}
\newcommand{\tmseven}{s}
\newcommand{\tmb}{u}  % b de bis plus pratique a ecrire
\newcommand{\tmbb}{v}  % 
\newcommand{\tmbbp}{v'}  % 

\newcommand{\bigtm}{M}
\newcommand{\bigtmtwo}{N}
\newcommand{\bigtmthree}{Q}
\newcommand{\bigtmfour}{R}
\newcommand{\bigtmfive}{P}

\newcommand{\var}{x}
\newcommand{\vartwo}{y}
\newcommand{\varthree}{z}
\newcommand{\varfour}{w}
\newcommand{\varp}{x'}
\newcommand{\vartwop}{y'}
\newcommand{\varthreep}{z'}
\newcommand{\varpp}{x''}
\newcommand{\vartwopp}{y''}
\newcommand{\varthreepp}{z''}

\newcommand{\mvar}{A}
\newcommand{\mvartwo}{B}
\newcommand{\mvarthree}{C}
\newcommand{\mvarfour}{D}


\newcommand{\varset}{\Delta}
\newcommand{\varsettwo}{\Gamma}
\newcommand{\varsetthree}{\Sigma}

\newcommand{\Var}{\tt Var}

\newcommand{\alpeq}{=_\alpha}

\newcommand{\ap}[2]{#1[#2]}
\renewcommand{\ap}[2]{#1#2}
\newcommand{\genap}[3]{#1[#2]\ldots[#3]}




%%%%%%%
%% REDUCIBILITY
%%%%%%%

\newcommand{\dist}{key}
\newcommand{\gir}{com}
\newcommand{\bse}{bs}
\newcommand{\todist}{\Rew{\dist}}
\newcommand{\todistalg}{\Rrightarrow_{\dist}}
\newcommand{\togir}{\Rew{\gir}}
\newcommand{\tobse}{\Rew{\bse}}
\newcommand{\sndist}{\sn{\dist}}
\newcommand{\snsubst}{\sn{\to}}

\newcommand{\redc}[1]{\llbracket#1\rrbracket}

\newcommand{\tree}{T}
\newcommand{\size}[1]{|#1|}
\newcommand{\sizep}[2]{|#1|_{#2}}
\newcommand{\sizem}[1]{\sizep{#1}{\msym}}
\newcommand{\sizee}[1]{\sizep{#1}{\esym}}
\newcommand{\sizedb}[1]{\sizep{#1}{\db}}
\newcommand{\sizels}[1]{\sizep{#1}{\lssym}}

\newcommand{\isubgen}[2]{\{\cdot\}_{#1}^{#2}}
\newcommand{\esubgen}[2]{[\cdot]_{#1}^{#2}}

\newcommand{\netson}[1]{nets_{#1}}
\newcommand{\netsontoprom}[1]{\netson{#1}^{\whyn}}
\newcommand{\netsA}{\netson{\form}}
\newcommand{\netsAtoprom}{\netson{\form}^{\whyn}}
\newcommand{\snA}{\sn{\form}}
\newcommand{\cutnet}[2]{cut(#1|#2)}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% CONTEXTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tarrow}[2]{#1 \rightarrow #2}
\newcommand{\ty}[2]{\tarrow{#1}{#2}}
\newcommand{\emptyctx}{\epsilon}
\newcommand{\typctx}{\Gamma}
\newcommand{\typctxtwo}{\Delta}
\newcommand{\typctxthree}{\Pi}




%%%%%%%%%%%%%%%%%
%%  STANDARDIZATION		%%
%%%%%%%%%%%%%%%%%

\newcommand{\deriv}{\ensuremath{d}}
\newcommand{\derivone}{\ensuremath{d}}
\newcommand{\derivtwo}{\ensuremath{e}}
\newcommand{\derivthree}{\ensuremath{f}}
\newcommand{\derivfour}{\ensuremath{g}}
\newcommand{\derivfive}{\ensuremath{h}}

\newcommand{\toover}[1]{\overset{#1}{\to}}
\newcommand{\toleft}{\Rew{leftmost}}

\newcommand{\nests}{\ensuremath{\prec}}
\newcommand{\nestsn}[1]{\ensuremath{\prec^{#1}}}
\newcommand{\nestsb}{\ensuremath{\prec_{\tt B}}}
\newcommand{\nestsEq}{\ensuremath{\preceq}}
\newcommand{\nestsbEq}{\ensuremath{\preceq_{\tt B}}}
\newcommand{\nestsbn}[1]{\ensuremath{\prec^{#1}_{\tt B}}}
\newcommand{\notnests}{\ensuremath{\nprec}}
\newcommand{\notnestsb}{\ensuremath{\nprec_{{{\tt B}}}}}
\newcommand{\notnestsEq}{\ensuremath{\npreceq}}
\newcommand{\notnestsbEq}{\ensuremath{\npreceq_{\tt B}}}
\newcommand{\nestsbone}{\ensuremath{\prec^1_{\tt B}}}
\newcommand{\nestsoned}{\ensuremath{\prec^1_d}}
\newcommand{\nestsone}{\ensuremath{\prec^1}}
\newcommand{\notnestsone}{\ensuremath{\nprec^1}}
\newcommand{\nestsonep}{\ensuremath{\prec^{1P}}}
\newcommand{\notnestsonep}{\ensuremath{\nprec^{1P}}}
\newcommand{\nestsoneo}{\ensuremath{\prec^{1O}}}

\newcommand{\unfsym}{\rotatebox[origin=c]{-90}{$\rightarrow$}}
\newcommand{\unf}[1]{#1\unfsym}
\newcommand{\relunf}[2]{\unf{#1}_{#2}}


%%%%%%%
%% LINEAR LAMBDA CALCULUS (WITH BANG)
%%%%%%%

\newcommand{\lb}{\l_!}

\newcommand{\tolsc}{\Rew{LSC}}
\newcommand{\rtom}{\mapsto_\msym}
\newcommand{\rtoe}{\mapsto_\esym}
\newcommand{\tom}{\Rew{\msym}}
\newcommand{\toe}{\Rew{\esym}}
\newcommand{\tow}{\Rew{\wsym}}
\newcommand{\wtom}{\Rew{\wsym\msym}}
\newcommand{\wtoe}{\Rew{\wsym\esym}}
\newcommand{\swtom}{\Rew{\ssym\wsym\msym}}
\newcommand{\swtoe}{\Rew{\ssym\wsym\esym}}

\newcommand{\tolb}{\Rew{\lb}}



%%%%%%%
%% LATEX SHORTCUTS
%%%%%%%
\newcommand{\ignore}[1]{}
\newcommand{\msep}{\hspace*{0.2cm}}
\newcommand{\sep}{\hspace*{0.5cm}}
\newcommand{\ms}{\medskip}
\newcommand{\bs}{\bigskip}
\newcommand{\mathintitle}[2]{\texorpdfstring{#1}{#2}}
\newcommand{\colspace}{@{\hspace{.5cm}}}
\newcommand{\myinput}[1]{\ifthenelse{\boolean{withimages}}{\input{#1}}{}}
\newcommand{\spc}{@{\hspace{.5cm}}}



\newcommand{\stratsym}{S}
\newcommand{\tostrat}{\Rew{\stratsym}}

\newcommand\Sysneutralvoid[1]{{#1}\mbox{-}neutral\xspace}
\newcommand\Sysnormalvoid[1]{{#1}\mbox{-}normal\xspace}
\newcommand\sysneutralvoid[1]{{#1}\mbox{-}neutral\xspace}
\newcommand\sysnormalvoid[1]{{#1}\mbox{-}normal\xspace}
\newcommand\sysnotabsvoid[1]{{#1}\mbox{-}abstraction\xspace}

\newcommand\sysnormalpr[1]{{\tt normal}_{#1}}
\newcommand\sysneutralpr[1]{{\tt neutral}_{#1}}
\newcommand\sysabspr[1]{{\tt abs}_{#1}}
\newcommand\sysnotabspr[1]{\neg \sysabspr{#1}}
\newcommand\sysnormal[2]{\sysnormalpr{#1}(#2)}
\newcommand\sysneutral[2]{\sysneutralpr{#1}(#2)}
\newcommand\sysabs[2]{\sysabspr{#1}(#2)}
\newcommand\sysnotabs[2]{\sysnotabspr{#1}(#2)}

\newcommand\spnormalpr{\sysnormalpr\spi}
\newcommand\spneutralpr{\sysneutralpr\spi}
\newcommand\spabspr{\sysabspr\spi}
\newcommand\spnotabspr{\sysnotabspr\spi}

\newcommand\spnormal[1]{\sysnormal\spi{#1}}
\newcommand\spneutral[1]{\sysneutral\spi{#1}}
\newcommand\spabs[1]{\sysabs\spi{#1}}
\newcommand\spnotabs[1]{\sysnotabs\spi{#1}}

\newcommand\system{\stratsym}
\newcommand\detsystem{det\stratsym}
\newcommand\systemem{\mem\mbox{-}\ske}
\newcommand\systemax{mx}
\newcommand\systemlh{\lh}
\newcommand\systemlsp{\lh}

\newcommand\neutype{\neutral}


\newcommand{\syssize}[2]{| #2|_{#1}}

% for references
\newcommand{\refappendix}[1]{Appendix~\ref{app:#1}}
\newcommand{\reflemma}[1]{Lemma~\ref{l:#1}}
\newcommand{\reflemmap}[2]{Lemma~\ref{l:#1}.\ref{p:#1-#2}}
\newcommand{\reflemmaeq}[1]{{L.\ref{l:#1}}}
\newcommand{\reflemmaeqp}[2]{{L.\ref{l:#1}.\ref{p:#1-#2}}}
\newcommand{\refcorollary}[1]{Corollary~\ref{c:#1}}
\newcommand{\refcorollaryp}[2]{Corollary~\ref{c:#1}.\ref{p:#1-#2}}
\newcommand{\refth}[1]{Theorem~\ref{th:#1}}
\newcommand{\refthp}[2]{Theorem~\ref{th:#1}.\ref{p:#1-#2}}
\newcommand{\refthm}[1]{Theorem~\ref{thm:#1}}
\newcommand{\refthmp}[2]{Theorem~\ref{thm:#1}.\ref{p:#1-#2}}
\newcommand{\reftm}[1]{Theorem~\ref{tm:#1}}
\newcommand{\reftmp}[2]{Theorem~\ref{tm:#1}.\ref{p:#1-#2}}
\newcommand{\refprop}[1]{Proposition~\ref{prop:#1}}
\newcommand{\refpropp}[2]{Proposition~\ref{prop:#1}.\ref{p:#1-#2}}
\newcommand{\refsect}[1]{Sect.~\ref{sect:#1}}
\newcommand{\refsubsect}[1]{Subsect.~\ref{subsect:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{sect:#1}}
\newcommand{\reftab}[1]{Table~\ref{tab:#1}}
\ifthenelse{\boolean{easychairstyle}}{}{
	%\newcommand{\refeq}[1]{(\ref{eq:#1})} %package mathtools defines \refeq, to solve 
}
\newcommand{\reffig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\refcoro}[1]{Corollary~\ref{coro:#1}}
\newcommand{\refcorop}[2]{Corollary~\ref{coro:#1}.\ref{p:#1-#2}}
\newcommand{\refdef}[1]{Definition~\ref{def:#1}}
\newcommand{\refdefp}[2]{Definition~\ref{def:#1}.\ref{p:#1-#2}}
\newcommand{\refrem}[1]{Remark~\ref{rem:#1}}
\newcommand{\refpoint}[1]{Point~\ref{p:#1}}
\newcommand{\refremark}[1]{Remark~\ref{rem:#1}}
\newcommand{\refsection}[1]{Section~\ref{s:#1}}

==> name-linear-anti-substitution.tex <==
% !TEX root = ../../main.tex
\begin{proof}
By induction on $\cbnctx$. Cases:
\begin{itemize}
  \item \emph{Empty context}, \ie $\cbnctx = \ctxhole$. Then $\tderiv \exder[\cbn] \Deri[(\msteps, \esteps)]{\typctx}{\tmtwo}{\type}$. And we simply take 
  \begin{itemize}
  \item $\tderiv_\tmtwo \defeq \tderiv$, that implies $\typetwo \defeq \type$, $\typctx_\tmtwo \defeq \typctx$, $\msteps_\tmtwo \defeq \msteps$, and $\esteps_\tmtwo \defeq \esteps$, and 
  \item $\tderiv_\var$ defined as the axiom 
  $$\infer[\ax]{\Deri[(0, 1)] {\var \col \single \type} \var \type}{} $$
  and for which $\typctx'$ is empty, $\msteps' = 0$, and $\esteps' = 1$. 
  \end{itemize}
  Then the statement holds:
  \begin{itemize}
  \item \emph{Typing contexts}: $\typctx = \emptyset \ctxplus \typctx = \emptyset \ctxplus  \typctx_\tmtwo = \typctx' \ctxplus  \typctx_\tmtwo$ and 
  \item \emph{Indices}: $(\msteps, \esteps) = (\msteps_{\tmtwo}, \esteps_{\tmtwo}) = (0 + \msteps_{\tmtwo}, 1 + \esteps_{\tmtwo} - 1) = (\msteps' + \msteps_{\tmtwo}, \esteps' + \esteps_{\tmtwo} - 1) $.
  \end{itemize}
  
  \item \emph{Left of an application}, \ie $\cbnctx = \cbnctxtwo \tmthree$. Then $\tderiv$ has the form
    $$\infer[\app]{
        \Deri[(\msteps_{\cbnctxtwop\tmtwo} + \msteps_\tmthree + 1, \esteps_{\cbnctxtwop\tmtwo} + \esteps_\tmthree)] {\typctx_{\cbnctxtwop\tmtwo} \ctxplus  \typctx_\tmthree}
             {\cbnctxtwop\tmtwo \tmthree} \type
      }{
        \tderiv_{\cbnctxtwop\tmtwo} \exder\Deri[(\msteps_{\cbnctxtwop\tmtwo}, \esteps_{\cbnctxtwop\tmtwo})] {\typctx_{\cbnctxtwop\tmtwo}} {\cbnctxtwop\tmtwo} {\ty{\mtype}{\type}}
        \quad
        \Deri[(\msteps_\tmthree, \esteps_\tmthree)] {\typctx_\tmthree} \tmthree {\mtype}
      }
      $$
  where $\typctx = \typctx_{\cbnctxtwop\tmtwo} \ctxplus \typctx_\tmthree$, $\msteps = \msteps_{\cbnctxtwop\tmtwo} + \msteps_\tmthree + 1$, and $\esteps = \esteps_{\cbnctxtwop\tmtwo} + \esteps_\tmthree$.
  
  Applying the \ih to $\tderiv_{\cbnctxtwop\tmtwo}$ provides a type $\typetwo$ and derivations:
  $$\tderiv_\tmtwo  \exder[\cbn] \Deri[(\msteps_\tmtwo, \esteps_\tmtwo)]{\typctx_\tmtwo}{\tmtwo}{\typetwo}$$
  and 
  $$\tderiv_{\cbnctxtwo\cwc{\var}} \exder[\cbn] 
 \Deri[(\mstepsthree, \estepsthree)]{  \typctx'' \ctxplus \var{:}\mult{\typetwo} }{\cbnctxtwo\cwc{\var}}{\ty{\mtype}{\type}}$$
  such that $\typctx_{\cbnctxtwop\tmtwo} = \typctx'' \ctxplus \typctx_\tmtwo$ and $(\msteps_{\cbnctxtwop\tmtwo}, \esteps_{\cbnctxtwop\tmtwo}) = (\mstepsthree +  \msteps_\tmtwo, \estepsthree + \esteps_\tmtwo- 1)$.
 
 Then $\tderiv_{\cbnctx\cwc{\var}}$ is given by: 
 $$\infer[\app]{
        \Deri[(\mstepsthree + \msteps_\tmthree + 1, \estepsthree + \esteps_\tmthree)] {\typctx'' \ctxplus \var{:}\mult{\typetwo} \ctxplus \typctx_\tmthree}
             {\cbnctxtwop\var \tmthree} \type
      }{
        \tderiv_{\cbnctxtwo\cwc{\var}} \exder[\cbn] 
 \Deri[(\mstepsthree, \estepsthree)]{  \typctx'' \ctxplus \var{:}\mult{\typetwo} }{\cbnctxtwo\cwc{\var}}{\ty{\mtype}{\type}}
        \quad
        \Deri[(\msteps_\tmthree, \esteps_\tmthree)] {\typctx_\tmthree} \tmthree {\mtype}
      }
      $$
  that, by taking $\typctx' \defeq \typctx'' \ctxplus \typctx_\tmthree$, $\mstepstwo = \mstepsthree + \msteps_\tmthree + 1$, and $\estepstwo = \estepsthree + \esteps_\tmthree$, verifies the statement because:
  \begin{itemize}
  \item \emph{Typing contexts}: $\typctx = \typctx_{\cbnctxtwop\tmtwo} \ctxplus \typctx_\tmthree = \typctx'' \ctxplus \typctx_\tmtwo \ctxplus \typctx_\tmthree = \typctx' \ctxplus \typctx_\tmtwo$, and 
  \item \emph{Indices}: $(\msteps, \esteps) = (\msteps_{\cbnctxtwop\tmtwo} + \msteps_\tmthree + 1, \esteps_{\cbnctxtwop\tmtwo} + \esteps_\tmthree) = (\mstepsthree +  \msteps_\tmtwo + \msteps_\tmthree + 1, \estepsthree + \esteps_\tmtwo- 1+ \esteps_\tmthree) = (\mstepstwo +  \msteps_\tmtwo, \estepstwo + \esteps_\tmtwo- 1)$.
  \end{itemize}
  
  \item \emph{Left of a substitution}, \ie $\cbnctx = \cbnctxtwo \esub\vartwo\tmthree$. Then $\tderiv$ has the form
    $$\infer[\esrule]{
        \Deri[(\msteps_{\cbnctxtwop\tmtwo} + \msteps_\tmthree, \esteps_{\cbnctxtwop\tmtwo} + \esteps_\tmthree)] {\typctx_{\cbnctxtwop\tmtwo} \ctxplus  \typctx_\tmthree}
             {\cbnctxtwop\tmtwo \esub\vartwo\tmthree} \type
      }{
        \tderiv_{\cbnctxtwop\tmtwo} \exder\Deri[(\msteps_{\cbnctxtwop\tmtwo}, \esteps_{\cbnctxtwop\tmtwo})] {\typctx_{\cbnctxtwop\tmtwo}; \vartwo:\mtype} {\cbnctxtwop\tmtwo} {\type}
        \quad
        \Deri[(\msteps_\tmthree, \esteps_\tmthree)] {\typctx_\tmthree} \tmthree {\mtype}
      }
      $$
  where $\typctx = \typctx_{\cbnctxtwop\tmtwo} \ctxplus  \typctx_\tmthree$, $\msteps = \msteps_{\cbnctxtwop\tmtwo} + \msteps_\tmthree$, and $\esteps = \esteps_{\cbnctxtwop\tmtwo} + \esteps_\tmthree$.
  
  Applying the \ih to $\tderiv_{\cbnctxtwop\tmtwo}$ provides a type $\typetwo$ and derivations:
  $$\tderiv_\tmtwo  \exder[\cbn] \Deri[(\msteps_\tmtwo, \esteps_\tmtwo)]{\typctx_\tmtwo}{\tmtwo}{\typetwo}$$
  and 
  $$\tderiv_{\cbnctxtwo\cwc{\var}} \exder[\cbn] 
 \Deri[(\mstepsthree, \estepsthree)]{  \typctx'';\vartwo:\mtype \ctxplus \var{:}\mult{\typetwo} }{\cbnctxtwo\cwc{\var}}{\type}$$
  such that $\typctx_{\cbnctxtwop\tmtwo} = \typctx'' \ctxplus  \typctx_\tmtwo$ and $(\msteps_{\cbnctxtwop\tmtwo}, \esteps_{\cbnctxtwop\tmtwo}) = (\mstepsthree +  \msteps_\tmtwo, \estepsthree + \esteps_\tmtwo- 1)$.
 
 Then $\tderiv_{\cbnctx\cwc{\var}}$ is given by: 
 $$\infer[\esrule]{
        \Deri[(\mstepsthree + \msteps_\tmthree , \estepsthree + \esteps_\tmthree)] {\typctx'' \ctxplus \var{:}\mult{\typetwo}  \ctxplus  \typctx_\tmthree}
             {\cbnctxtwop\var \esub\vartwo\tmthree} \type
      }{
        \tderiv_{\cbnctxtwo\cwc{\var}} \exder[\cbn] 
 \Deri[(\mstepsthree, \estepsthree)]{  \typctx'';\vartwo:\mtype \ctxplus \var{:}\mult{\typetwo} }{\cbnctxtwo\cwc{\var}}{\type}
        \quad
        \Deri[(\msteps_\tmthree, \esteps_\tmthree)] {\typctx_\tmthree} \tmthree {\mtype}
      }
      $$
  that, by taking $\typctx' \defeq \typctx'' \ctxplus  \typctx_\tmthree$, $\mstepstwo = \mstepsthree + \msteps_\tmthree$, and $\estepstwo = \estepsthree + \esteps_\tmthree$, verifies the statement because:
  \begin{itemize}
  \item \emph{Typing contexts}: $\typctx = \typctx_{\cbnctxtwop\tmtwo} \ctxplus  \typctx_\tmthree = \typctx'' \ctxplus  \typctx_\tmtwo \ctxplus  \typctx_\tmthree $, and 
  \item \emph{Indices}: $(\msteps, \esteps) = (\msteps_{\cbnctxtwop\tmtwo} + \msteps_\tmthree, \esteps_{\cbnctxtwop\tmtwo} + \esteps_\tmthree) = (\mstepsthree +  \msteps_\tmtwo + \msteps_\tmthree, \estepsthree + \esteps_\tmtwo- 1+ \esteps_\tmthree) = (\mstepstwo +  \msteps_\tmtwo, \estepstwo + \esteps_\tmtwo- 1)$.\qed
  \end{itemize}
\end{itemize}

\end{proof}

==> value-linear-substitution-bis.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By induction on $\cbvctx$.
	Cases:
	\begin{itemize}
		\item \emph{Hole}, \ie $\cbvctx = \ctxhole$, then $\cbvctx\cwc{\val} = \val$ and $\cbvctx\cwc{\var} = \var$, hence $\tderiv$ consists only of an $\ax$-rule and so $\mtypetwo = \mtype$ and $\dom{\typctx} = \emptyset$, with $\msteps = 0$ and $\esteps = 1$.
		Let $\mtypethree \defeq \mtype$ and $\mtypefour \defeq \emptymset$.
		Thus, for every $\tderivtwo\exder[\cbvsym] \Deri[(\mstepstwo, \estepstwo)]{\typctxtwo}{\val}{\mtypethree}$, one has $\dom{\typctxtwo} = \emptyset$ and $\mstepstwo = 0 = \estepstwo$ by \reflemmap{value-typing}{empty}.
		Hence, $\tderivtwo$ coincides with a derivation $\tderiv' \exder[\cbvsym] \Deri[(\msteps+\mstepstwo, \esteps+\estepstwo - 1)]{\typctx \mplus \typctxtwo, \var \col \mtypefour}{\cbvctx\cwc{\val}}{\mtypetwo}$.

		\item \emph{Left application}, \ie $\cbvctx \defeq \cbvctxtwo\tm$.
		Then, the type derivation $\tderiv$ has the form
		\begin{equation*}
				\infer[\app]{
			\Deri[(\msteps, \esteps)] {\var \col \mtype, \typctx}
			{\cbvctxtwo\cwc{\var}\tm} \mtypetwo
		}{
			\Deri[(\msteps_{1}, \esteps_{1})] {\var \col \mtype_{1}, \typctx_{1}} {\cbvctxtwo\cwc{\var}} {\single{\ty{\mtypetwo'}{\mtypetwo}}}
			\qquad
			\Deri[(\msteps_{2}, \esteps_{2})] {\var \col \mtype_{2}, \typctx_{2}} \tm {\mtypetwo'}
		}
		\end{equation*}
		
		where $\mtype = \mtype_{1} \mplus \mtype_{2}$, $\typctx = \typctx_{1} \mplus \typctx_{2}$, $\msteps = \msteps_{1} + \msteps_{2} + 1$ and $\esteps = \esteps_{1} + \esteps_{2}$.
		By \ih, there exists a splitting $\mtype_{1} = \mtypethree \mplus \mtypefour'$ such that, for every derivation $\tderivtwo \exder[\cbvsym] \Deri[(\mstepstwo,\estepstwo)]{\typctxtwo}{\val}{\mtypethree}$, there is a derivation of $\Deri[(\msteps_{1}+\mstepstwo, \esteps_{1}+\estepstwo-1)]{\typctx_{1} \mplus \typctxtwo, \var \col \mtypefour'}{\cbvctxtwo\cwc{\val}}{\single{\ty{\mtypetwo'}{\mtypetwo}}}$.
		So, we have the derivation $\tderiv'$
		\begin{equation*}
		\infer[\app]{
			\Deri[(\msteps+\mstepstwo, \esteps + \estepstwo-1)] {\var \col \mtype_{\typctxthree} \mplus \mtypefour', \typctx \mplus \typctxtwo}
			{\cbvctxtwo\cwc{\val}\tm} \mtypetwo
		}{
			\Deri[(\msteps_{1}+\mstepstwo, \esteps_{1}+\estepstwo-1)]{\typctx_{1} \mplus \typctxtwo, \var \col \mtypefour'}{\cbvctxtwo\cwc{\val}}{\single{\ty{\mtypetwo'}{\mtypetwo}}}
			\qquad
			\Deri[(\msteps_{2}, \esteps_{2})] {\var \col \mtype_{2}, \typctx_2} \tm {\mtypetwo'}
		}
		\end{equation*}
		where $\mtypefour \defeq \mtype_{1} \mplus \mtypefour'$ and $\mtype = \mtype_{1} \mplus \mtype_{2} = \mtypethree \mplus \mtypefour' \mplus \mtype_{2} = \mtypethree \mplus \mtypefour$.
	
		
		\item \emph{Right application}, \ie $\cbvctx \defeq \valtwo\cbvctxtwo$.
		Then, the type derivation $\tderiv$ has the form
		\begin{equation*}
		\infer[\app]{
			\Deri[(\msteps, \esteps)] {\var \col \mtype, \typctx}
			{\valtwo\,\cbvctxtwo\cwc{\var}} \mtypetwo
		}{
			\Deri[(\msteps_1, \esteps_1)] {\var \col \mtype_1, \typctx_1} {\valtwo} {\single{\ty{\mtypetwo'}{\mtypetwo}}}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} {\cbvctxtwo\cwc{\var}} {\mtypetwo'}
		}
		\end{equation*}
		where $\mtype = \mtype_1 \mplus \mtype_2$, $\typctx = \typctx_1 \mplus \typctx_2$, $\msteps = \msteps_1 + \msteps_2 + 1$ and $\esteps = \esteps_1 + \esteps_2$.
		By \ih, there is a splitting $\mtype_{2} = \mtypethree \mplus \mtypefour'$ such that, for every derivation $\tderivtwo \exder[\cbvsym] \Deri[(\mstepstwo,\estepstwo)]{\typctxtwo}{\val}{\mtypethree}$, there is a derivation of $\Deri[(\msteps_{2}+\mstepstwo, \esteps_{2}+\estepstwo-1)]{\typctx_2 \mplus \typctxtwo, \var \col \mtypefour'}{\cbvctxtwo\cwc{\val}}{\mtypetwo'}$.
		So, we have the derivation $\tderiv'$
		\begin{equation*}
		\infer[\app]{
			\Deri[(\msteps+\mstepstwo, \esteps + \estepstwo-1)] {\var \col \mtype_{1} \mplus \mtypefour', \typctx \mplus \typctxtwo}
			{\valtwo\cbvctxtwo\cwc{\val}} \mtypetwo
		}{
			\Deri[(\msteps_{1}, \esteps_{1})] {\var \col \mtype_{1}, \typctx_{1}} {\valtwo} {\single{\ty{\mtypetwo'}{\mtypetwo}}}
			\qquad
			\Deri[(\msteps_{2}+\mstepstwo, \esteps_{2}+\estepstwo-1)]{\typctx_{2} \mplus \typctxtwo, \var \col \mtypefour'}{\cbvctxtwo\cwc{\val}}{\mtypetwo'}
		}
		\end{equation*}
		where $\mtypefour \defeq \mtype_{1} \mplus \mtypefour'$ and $\mtype = \mtype_{1} \mplus \mtype_{2} = \mtype_{1} \mplus \mtypethree \mplus \mtypefour' = \mtypethree \mplus \mtypefour$.
	
		\item \emph{Left explicit substitution}, \ie $\cbvctx \defeq \cbvctxtwo\esub{\vartwo}\tm$ where $\tm \defeq \sctxp{\valtwo}$.
		We can suppose without loss of generality that $\vartwo \notin \fv{\tm} \cup \fv{\val} \cup \{ \var\}$, in particular $\vartwo \notin \dom{\typctxtwo}$.
		So, the type derivation $\tderiv$ has the form
		\begin{equation*}
		\infer[\esrule]{
			\Deri[(\msteps, \esteps)] {\var \col \mtype, \typctx}
			{\cbvctxtwo\cwc{\var}\esub{\vartwo}\tm} \mtypetwo
		}{
			\Deri[(\msteps_1, \esteps_1)] {\var \col \mtype_1, \vartwo \col{\mtypetwo'}, \typctx_1} {\cbvctxtwo\cwc{\var}} {\mtypetwo}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} \tm {\mtypetwo'}
		}
		\end{equation*}
		where $\mtype = \mtype_1 \mplus \mtype_2$, $\typctx = \typctx_1 \mplus \typctx_2$, $\msteps = \msteps_1 + \msteps_2$ and $\esteps = \esteps_1 + \esteps_2$.
		By \ih, there exists a splitting $\mtype_{1} = \mtypethree \mplus \mtypefour'$ such that, for every derivation $\tderivtwo \exder[\cbvsym] \Deri[(\mstepstwo,\estepstwo)]{\typctxtwo}{\val}{\mtypethree}$, there is a derivation of $\Deri[(\msteps_{1}+\mstepstwo, \esteps_{1}+\estepstwo-1)]{\typctx_{1} \mplus \typctxtwo, \var \col \mtypefour', \vartwo \col \mtypetwo'}{\cbvctxtwo\cwc{\val}}{\mtypetwo}$.
		So, we have the derivation $\tderiv'$
		\begin{equation*}
		\infer[\esrule]{
			\Deri[(\msteps+\mstepstwo, \esteps + \estepstwo-1)] {\var \col \mtype_{\typctxthree} \mplus \mtypefour', \typctx \mplus \typctxtwo}
			{\cbvctxtwo\cwc{\val}\esub{\vartwo}\tm} \mtypetwo
		}{
			\Deri[(\msteps_{1}+\mstepstwo, \esteps_{1}+\estepstwo-1)]{\typctx_{1} \mplus \typctxtwo, \var \col \mtypefour', \vartwo \col \mtypetwo'}{\cbvctxtwo\cwc{\val}}{\mtypetwo}
			\qquad
			\Deri[(\msteps_{2}, \esteps_{2})] {\var \col \mtype_{2}, \typctx_2} \tm {\mtypetwo'}
		}
		\end{equation*}
		where $\mtypefour \defeq \mtype_{1} \mplus \mtypefour'$ and $\mtype = \mtype_{1} \mplus \mtype_{2} = \mtypethree \mplus \mtypefour' \mplus \mtype_{2} = \mtypethree \mplus \mtypefour$.
		
		\item \emph{Right explicit substitution}, \ie $\cbvctx \defeq \valtwo\esub{\vartwo}\cbvctxtwo$.
		We can suppose without loss of generality that $\vartwo \notin \fv{\val} \cup \{ \var\}$, in particular $\vartwo \notin \dom{\typctxtwo}$.
		Then, the type derivation $\tderiv$ has the form
		\begin{equation*}
		\infer[\esrule]{
			\Deri[(\msteps, \esteps)] {\var \col \mtype, \typctx}
			{\valtwo\esub{\vartwo}{\cbvctxtwo\cwc{\var}}} \mtypetwo
		}{
			\Deri[(\msteps_1, \esteps_1)] {\var \col \mtype_1, \vartwo \col \mtypetwo', \typctx_1} {\valtwo} {\mtypetwo}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} {\cbvctxtwo\cwc{\var}} {\mtypetwo'}
		}
		\end{equation*}
		where $\mtype = \mtype_1 \mplus \mtype_2$, $\typctx = \typctx_1 \mplus \typctx_2$, $\msteps = \msteps_1 + \msteps_2$ and $\esteps = \esteps_1 + \esteps_2$.
		By \ih, there is a splitting $\mtype_{2} = \mtypethree \mplus \mtypefour'$ such that, for every derivation $\tderivtwo \exder[\cbvsym] \Deri[(\mstepstwo,\estepstwo)]{\typctxtwo}{\val}{\mtypethree}$, there is a derivation of $\Deri[(\msteps_{2}+\mstepstwo, \esteps_{2}+\estepstwo-1)]{\typctx_2 \mplus \typctxtwo, \var \col \mtypefour'}{\cbvctxtwo\cwc{\val}}{\mtypetwo'}$.
		So, we have the derivation $\tderiv'$
		\begin{equation*}
		\infer[\esrule]{
			\Deri[(\msteps+\mstepstwo, \esteps + \estepstwo-1)] {\var \col \mtype_{1} \mplus \mtypefour', \typctx \mplus \typctxtwo}
			{\valtwo\cbvctxtwo\cwc{\val}} \mtypetwo
		}{
			\Deri[(\msteps_{1}, \esteps_{1})] {\var \col \mtype_{1}, \vartwo \col \mtypetwo', \typctx_{1}} {\valtwo} {\mtypetwo}
			\qquad
			\Deri[(\msteps_{2}+\mstepstwo, \esteps_{2}+\estepstwo-1)]{\typctx_{2} \mplus \typctxtwo, \var \col \mtypefour'}{\cbvctxtwo\cwc{\val}}{\mtypetwo'}
		}
		\end{equation*}
		where $\mtypefour \defeq \mtype_{1} \mplus \mtypefour'$ and $\mtype = \mtype_{1} \mplus \mtype_{2} = \mtype_{1} \mplus \mtypethree \mplus \mtypefour' = \mtypethree \mplus \mtypefour$.
	\end{itemize}
\end{proof}



==> value-linear-substitution.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By induction on $\cbvctx$.
	Cases:
	\begin{itemize}
		\item \emph{Hole}, \ie $\cbvctx = \ctxhole$, then $\cbvctx\cwc{\val} = \val$ and $\cbvctx\cwc{\var} = \var$, hence $\tderiv$ consists only of an $\ax$-rule and so $\mtypetwo = \mtype$ and $\dom{\typctx} = \emptyset$, with $\msteps = 0$ and $\esteps = 1$.
		Let $\mtype_1 \defeq \mtype$, $\mtype_2 \defeq \emptymset$, $\typctxtwo_1 \defeq \typctxtwo$ and $\typctxtwo_2$ be such that $\dom{\typctxtwo_2} = \emptyset$; also, we set $\msteps_1 \defeq \mstepstwo$, $\esteps_1 \defeq \estepstwo$ and $\msteps_2 \defeq 0 \eqdef \esteps_2$: then $\mtypetwo = \mtype = \mtype_1 \uplus \mtype_2$ and $\typctxtwo = \typctxtwo_1 \uplus \typctxtwo_2$, thus the conclusion of the type derivation $\tderivtwo$ can be seen as both $\Deri[(\msteps_1, \esteps_1)]{\typctxtwo_1}{\val}{\mtype_1}$ and $\Deri[(\msteps+\msteps_1, \esteps + \esteps_1-1)]{\var:\mtype_2,  \typctx \mplus \typctxtwo_1}{\cbvctx\cwc{\val}}{\mtypetwo}$ (since $\msteps_1 = \msteps + \msteps_1$ and $\esteps_1 = \esteps + \esteps_1 - 1$).
		Moreover, $\Deri[(\msteps_2, \esteps_2)]{\typctxtwo_2}{\val}{\mtype_2}$ is derivable by \reflemmap{value-typing}{judg}, and $\mstepstwo = \msteps_1 + \msteps_2$ and $\estepstwo = \esteps_1 + \esteps_2$.

		\item \emph{Left application}, \ie $\cbvctx \defeq \cbvctxtwo\tm$.
		Then, the type derivation $\tderiv$ has the form
		\begin{equation*}
				\infer[\app]{
			\Deri[(\msteps, \esteps)] {\var \col \mtype, \typctx}
			{\cbvctxtwo\cwc{\var}\tm} \mtypetwo
		}{
			\Deri[(\msteps_1, \esteps_1)] {\var \col \mtype_1, \typctx_1} {\cbvctxtwo\cwc{\var}} {\single{\ty{\mtypethree}{\mtypetwo}}}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} \tm {\mtypethree}
		}
		\end{equation*}
		where $\mtype = \mtype_1 \mplus \mtype_2$, $\typctx = \typctx_1 \mplus \typctx_2$, $\msteps = \msteps_1 + \msteps_2 + 1$ and $\esteps = \esteps_1 + \esteps_2$.
		By multiset splitting (\reflemmap{value-typing}{dec}) there are type derivations $\tderivtwo_1 \exder[\cbv] \Deri[(\mstepstwo_1,\estepstwo_1)]{\typctxtwo_1}{\val}{\mtype_1}$ and		$\tderivtwo_2 \exder[\cbv]\Deri[(\mstepstwo_2,\estepstwo_2)]{\typctxtwo_2}{\val}{\mtype_2}$ such that $\typctxtwo = \typctxtwo_1 \uplus \typctxtwo_2$, $\mstepstwo = \mstepstwo_1 +  \mstepstwo_2$ and $\estepstwo = \estepstwo_1 +  \estepstwo_2$.
		By \ih, $\esteps_1 \geq 1$ (and hence $\esteps \geq 1$) and there are splittings $\mtype_1 = \mtype_{11} \mplus \mtype_{12}$ and $\typctxtwo_1 = \typctxtwo_{11} \mplus \typctxtwo_{12}$ such that the judgements $\Deri[(\mstepstwo_{11}, \estepstwo_{11})]{\typctxtwo_{11}}{\val}{\mtype_{11}}$ and $\Deri[(\mstepstwo_{12}, \estepstwo_{12})]{\typctxtwo_{12}}{\val}{\mtype_{12}}$ and $\Deri[(\msteps_1+\mstepstwo_{11}, \esteps_1 + \estepstwo_{11}-1)]{\var \col \mtype_{12}, \typctx_1 \mplus \typctxtwo_{11}}{\cbvctxtwo\cwc{\val}}{\single{\ty{\mtypethree}\mtypetwo}}$ are derivable, with $\mstepstwo_1 = \mstepstwo_{11} + \mstepstwo_{12}$ and $\estepstwo_1 = \estepstwo_{11} + \estepstwo_{12}$.
		So, we have the type derivation
		\begin{equation*}
		\infer[\app]{
			\Deri[(\msteps+\mstepstwo_{11}, \esteps + \estepstwo_{11}-1)] {\var \col \mtype_{12} \mplus \mtype_2, \typctx \mplus \typctxtwo_{11}}
			{\cbvctxtwo\cwc{\val}\tm} \mtypetwo
		}{
			\Deri[(\msteps_1+\mstepstwo_{11}, \esteps_1 + \estepstwo_{11}-1)]{\var \col \mtype_{12}, \typctx_1 \mplus \typctxtwo_{11}}{\cbvctxtwo\cwc{\val}}{\single{\ty{\mtypethree}\mtypetwo}}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} \tm {\mtypethree}
		}
		\end{equation*}		
		where $\mtype = \mtype_{11} \mplus (\mtype_{12} \mplus \mtype_2)$.
		By multiset merging (\reflemmap{value-typing}{merg}), the judgement $\Deri[(\mstepstwo_{12}+\mstepstwo_2,\estepstwo_{12}+\estepstwo_2)]{\typctxtwo_{12} \mplus \typctxtwo_2}{\val}{\mtype_{12} \mplus \mtype_2}$ is derivable, with $\mstepstwo = \mstepstwo_1 + \mstepstwo_2 = \mstepstwo_{11} + (\mstepstwo_{12} + \mstepstwo_2)$ and $\estepstwo = \estepstwo_1 + \estepstwo_2 = \estepstwo_{11} + (\estepstwo_{12} + \estepstwo_2)$.
		
		\item \emph{Right application}, \ie $\cbvctx \defeq \valtwo\cbvctxtwo$.
		Then, the type derivation $\tderiv$ has the form
		\begin{equation*}
		\infer[\app]{
			\Deri[(\msteps, \esteps)] {\var \col \mtype, \typctx}
			{\valtwo\,\cbvctxtwo\cwc{\var}} \mtypetwo
		}{
			\Deri[(\msteps_1, \esteps_1)] {\var \col \mtype_1, \typctx_1} {\valtwo} {\single{\ty{\mtypethree}{\mtypetwo}}}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} {\cbvctxtwo\cwc{\var}} {\mtypethree}
		}
		\end{equation*}
		where $\mtype = \mtype_1 \mplus \mtype_2$, $\typctx = \typctx_1 \mplus \typctx_2$, $\msteps = \msteps_1 + \msteps_2 + 1$ and $\esteps = \esteps_1 + \esteps_2$.
		By multiset splitting (\reflemmap{value-typing}{dec}) there are type derivations $\tderivtwo_1 \exder[\cbv] \Deri[(\mstepstwo_1,\estepstwo_1)]{\typctxtwo_1}{\val}{\mtype_1}$ and		$\tderivtwo_2 \exder[\cbv]\Deri[(\mstepstwo_2,\estepstwo_2)]{\typctxtwo_2}{\val}{\mtype_2}$ such that $\typctxtwo = \typctxtwo_1 \uplus \typctxtwo_2$, $\mstepstwo = \mstepstwo_1 +  \mstepstwo_2$ and $\estepstwo = \estepstwo_1 +  \estepstwo_2$.
		By \ih, $\esteps_2 \geq 1$ (and hence $\esteps \geq 1$) and there are splittings $\mtype_2 = \mtype_{21} \mplus \mtype_{22}$ and $\typctxtwo_2 = \typctxtwo_{21} \mplus \typctxtwo_{22}$ such that the judgements $\Deri[(\mstepstwo_{21}, \estepstwo_{21})]{\typctxtwo_{21}}{\val}{\mtype_{21}}$ and $\Deri[(\mstepstwo_{22}, \estepstwo_{22})]{\typctxtwo_{22}}{\val}{\mtype_{22}}$ and $\Deri[(\msteps_2+\mstepstwo_{21}, \esteps_2 + \estepstwo_{21}-1)]{\var \col \mtype_{22}, \typctx_2 \mplus \typctxtwo_{21}}{\cbvctxtwo\cwc{\val}}{\mtypethree}$ are derivable, with $\mstepstwo_2 = \mstepstwo_{21} + \mstepstwo_{22}$ and $\estepstwo_2 = \estepstwo_{21} + \estepstwo_{22}$.
		So, we have the type derivation
		\begin{equation*}
		\infer[\app]{
			\Deri[(\msteps+\mstepstwo_{21}, \esteps + \estepstwo_{21}-1)] {\var \col \mtype_1 \mplus \mtype_{22}, \typctx \mplus \typctxtwo_{21}}
			{\valtwo \, \cbvctxtwo\cwc{\val}} \mtypetwo
		}{
			\Deri[(\msteps_1, \esteps_1)] {\var \col \mtype_1, \typctx_1} {\valtwo} {\single{\ty{\mtypethree}{\mtypetwo}}}
			\qquad
			\Deri[(\msteps_2+\mstepstwo_{21}, \esteps_2 + \estepstwo_{21}-1)]{\var \col \mtype_{22}, \typctx_2 \mplus \typctxtwo_{21}}{\cbvctxtwo\cwc{\val}}{\mtypethree}
		}
		\end{equation*}		
		where $\mtype = (\mtype_1 \mplus \mtype_{22}) \mplus \mtype_{21}$.
		By multiset merging (\reflemmap{value-typing}{merg}), the judgement $\Deri[(\mstepstwo_{1}+\mstepstwo_{22},\estepstwo_{1}+\estepstwo_{22})]{\typctxtwo_{1} \mplus \typctxtwo_{22}}{\val}{\mtype_{1} \mplus \mtype_{22}}$ is derivable, with $\mstepstwo = \mstepstwo_1 + \mstepstwo_2 = (\mstepstwo_{1} + \mstepstwo_{22}) + \mstepstwo_{21}$ and $\estepstwo = \estepstwo_1 + \estepstwo_2 = (\estepstwo_{1} + \estepstwo_{22}) + \estepstwo_{21}$.
		
		\item \emph{Left explicit substitution}, \ie $\cbvctx \defeq \cbvctxtwo\esub{\vartwo}\tm$.
		We can suppose without loss of generality that $\vartwo \notin \fv{\tm} \cup \fv{\val} \cup \{ \var\}$, in particular $\vartwo \notin \dom{\typctxtwo}$.
		So, the type derivation $\tderiv$ has the form
		\begin{equation*}
		\infer[\esrule]{
			\Deri[(\msteps, \esteps)] {\var \col \mtype, \typctx}
			{\cbvctxtwo\cwc{\var}\esub{\vartwo}\tm} \mtypetwo
		}{
			\Deri[(\msteps_1, \esteps_1)] {\var \col \mtype_1, \vartwo \col{\mtypethree}, \typctx_1} {\cbvctxtwo\cwc{\var}} {\mtypetwo}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} \tm {\mtypethree}
		}
		\end{equation*}
		where $\mtype = \mtype_1 \mplus \mtype_2$, $\typctx = \typctx_1 \mplus \typctx_2$, $\msteps = \msteps_1 + \msteps_2$ and $\esteps = \esteps_1 + \esteps_2$.
		By multiset splitting (\reflemmap{value-typing}{dec}) there are type derivations $\tderivtwo_1 \exder[\cbv] \Deri[(\mstepstwo_1,\estepstwo_1)]{\typctxtwo_1}{\val}{\mtype_1}$ and		$\tderivtwo_2 \exder[\cbv]\Deri[(\mstepstwo_2,\estepstwo_2)]{\typctxtwo_2}{\val}{\mtype_2}$ such that $\typctxtwo = \typctxtwo_1 \uplus \typctxtwo_2$, $\mstepstwo = \mstepstwo_1 +  \mstepstwo_2$ and $\estepstwo = \estepstwo_1 +  \estepstwo_2$.
		By \ih, $\esteps_1 \geq 1$ (and hence $\esteps \geq 1$) and there are splittings $\mtype_1 = \mtype_{11} \mplus \mtype_{12}$ and $\typctxtwo_1 = \typctxtwo_{11} \mplus \typctxtwo_{12}$ such that the judgements $\Deri[(\mstepstwo_{11}, \estepstwo_{11})]{\typctxtwo_{11}}{\val}{\mtype_{11}}$ and $\Deri[(\mstepstwo_{12}, \estepstwo_{12})]{\typctxtwo_{12}}{\val}{\mtype_{12}}$ and $\Deri[(\msteps_1+\mstepstwo_{11}, \esteps_1 + \estepstwo_{11}-1)]{\var \col \mtype_{12}, \vartwo \col \mtypethree, \typctx_1 \mplus \typctxtwo_{11}}{\cbvctxtwo\cwc{\val}}{\mtypetwo}$ are derivable, with $\mstepstwo_1 = \mstepstwo_{11} + \mstepstwo_{12}$ and $\estepstwo_1 = \estepstwo_{11} + \estepstwo_{12}$.
		Thus, we have the type derivation
		\begin{equation*}
		\infer[\esrule]{
			\Deri[(\msteps+\mstepstwo_{11}, \esteps + \estepstwo_{11}-1)] {\var \col \mtype_{12} \mplus \mtype_2, \typctx \mplus \typctxtwo_{11}}
			{\cbvctxtwo\cwc{\val}\tm} \mtypetwo
		}{
			\Deri[(\msteps_1+\mstepstwo_{11}, \esteps_1 + \estepstwo_{11}-1)]{\var \col \mtype_{12}, \vartwo \col \mtypethree, \typctx_1 \mplus \typctxtwo_{11}}{\cbvctxtwo\cwc{\val}}{\mtypetwo}
			\qquad
			\Deri[(\msteps_2, \esteps_2)] {\var \col \mtype_2, \typctx_2} \tm {\mtypethree}
		}
		\end{equation*}		
		where $\mtype = \mtype_{11} \mplus (\mtype_{12} \mplus \mtype_2)$.
		By multiset merging (\reflemmap{value-typing}{merg}), the judgement $\Deri[(\mstepstwo_{12}+\mstepstwo_2,\estepstwo_{12}+\estepstwo_2)]{\typctxtwo_{12} \mplus \typctxtwo_2}{\val}{\mtype_{12} \mplus \mtype_2}$ is derivable, with $\mstepstwo = \mstepstwo_1 + \mstepstwo_2 = \mstepstwo_{11} + (\mstepstwo_{12} + \mstepstwo_2)$ and $\estepstwo = \estepstwo_1 + \estepstwo_2 = \estepstwo_{11} + (\estepstwo_{12} + \estepstwo_2)$.
\qed
	\end{itemize}
\end{proof}


